MARVEL: Multimodal Adaptive Reasoning-intensiVe Expand-rerank and retrievaL

Multimodal retrieval over text corpora remains a fundamental challenge: the best vision-language encoder achieves only 27.6 nDCG@10 on MM-BRIGHT, a reasoning-intensive multimodal retrieval benchmark, underperforming strong text-only systems. We argue that effective multimodal retrieval requires three tightly integrated capabilities that existing approaches address only in isolation: expanding the query's latent intent, retrieving with a model trained for complex reasoning, and reranking via explicit step-by-step reasoning over candidates. We introduce \textbf{MARVEL} (\textbf{M}ultimodal \textbf{A}daptive \textbf{R}easoning-intensi\textbf{V}e \textbf{E}xpand-rerank and retrieva\textbf{L}), a unified pipeline that combines LLM-driven query expansion, \textbf{MARVEL-Retriever} -- a reasoning-enhanced dense retriever fine-tuned for complex multimodal queries -- and GPT-4o-based chain-of-thought reranking with optional multi-pass reciprocal rank fusion. Evaluated on MM-BRIGHT across 29 technical domains, MARVEL achieves \textbf{37.9} nDCG@10, surpassing the best multimodal encoder by \textbf{+10.3 points} and outperforming all single-stage baselines in 27 of 29 domains and matching or approaching the best baseline in the remaining two highly-specialized domains (Crypto, Quantum Computing), demonstrating that reasoning-intensive multimodal retrieval is best addressed through a unified expand-retrieve-rerank framework. https://github.com/mm-bright/multimodal-reasoning-retrieval

==> reference.tex <==
% ============================================================
% CORE RETRIEVAL
% ============================================================

@inproceedings{karpukhin2020dpr,
  title     = {Dense Passage Retrieval for Open-Domain Question Answering},
  author    = {Karpukhin, Vladimir and O{\u{g}}uz, Barlas and Min, Sewon and
               Lewis, Patrick and Wu, Ledell and Edunov, Sergey and
               Chen, Danqi and Yih, Wen-tau},
  booktitle = {Proceedings of EMNLP},
  pages     = {6769--6781},
  year      = {2020}
}

@inproceedings{reimers2019sentence,
  title     = {Sentence-{BERT}: Sentence Embeddings using {Siamese BERT}-Networks},
  author    = {Reimers, Nils and Gurevych, Iryna},
  booktitle = {Proceedings of EMNLP},
  year      = {2019}
}

@article{ni2022large,
  title   = {Large Dual Encoders Are Generalizable Retrievers},
  author  = {Ni, Jianmo and Qu, Chen and Lu, Jing and Dai, Zhuyun and
             {\'A}brego, Gustavo Hern{\'a}ndez and Ma, Ji and Zhao, Vincent
             and Luan, Yi and Hall, Keith and Chang, Ming-Wei and Mei, Qiaozhu},
  journal = {arXiv preprint arXiv:2112.07899},
  year    = {2022}
}

@inproceedings{johnson2019faiss,
  title     = {Billion-Scale Similarity Search with {GPU}s},
  author    = {Johnson, Jeff and Douze, Matthijs and J{\'e}gou, Herv{\'e}},
  journal   = {IEEE Transactions on Big Data},
  volume    = {7},
  pages     = {535--547},
  year      = {2019}
}

@inproceedings{thakur2021beir,
  title     = {{BEIR}: A Heterogeneous Benchmark for Zero-shot Evaluation of
               Information Retrieval Models},
  author    = {Thakur, Nandan and Reimers, Nils and R{\"u}ckl{\'e}, Andreas and
               Srivastava, Abhishek and Gurevych, Iryna},
  booktitle = {Proceedings of NeurIPS Datasets and Benchmarks},
  year      = {2021}
}

@article{muennighoff2023mteb,
  title   = {{MTEB}: Massive Text Embedding Benchmark},
  author  = {Muennighoff, Niklas and Tazi, Nouamane and Magne, Lo{\"\i}c and
             Reimers, Nils},
  journal = {arXiv preprint arXiv:2210.07316},
  year    = {2023}
}

@inproceedings{robertson2009bm25,
  title     = {The Probabilistic Relevance Framework: {BM25} and Beyond},
  author    = {Robertson, Stephen and Zaragoza, Hugo},
  journal   = {Foundations and Trends in Information Retrieval},
  volume    = {3},
  number    = {4},
  pages     = {333--389},
  year      = {2009}
}

% ============================================================
% RAG / KNOWLEDGE-INTENSIVE
% ============================================================

@inproceedings{lewis2020rag,
  title     = {Retrieval-Augmented Generation for Knowledge-Intensive {NLP} Tasks},
  author    = {Lewis, Patrick and Perez, Ethan and Piktus, Aleksandra and
               Petroni, Fabio and Karpukhin, Vladimir and Goyal, Naman and
               K{\"u}ttler, Heinrich and Lewis, Mike and Yih, Wen-tau and
               Rockt{\"a}schel, Tim and Riedel, Sebastian and Kiela, Douwe},
  booktitle = {Advances in Neural Information Processing Systems},
  volume    = {33},
  pages     = {9459--9474},
  year      = {2020}
}

% ============================================================
% BENCHMARKS
% ============================================================

@article{su2025bright,
  title   = {{BRIGHT}: A Realistic and Challenging Benchmark for
             Reasoning-Intensive Retrieval},
  author  = {Su, Hongjin and Yen, Howard and Xia, Mengzhou and Shi, Weijia and
             Muennighoff, Niklas and Wang, Han-yu and Liu, Haisu and Shi, Quan
             and Siegel, Zachary S. and Tang, Michael and Sun, Ruoxi and Yoon,
             Jinsung and Arik, Sercan {\"O}. and Chen, Danqi and Yu, Tao},
  journal = {arXiv preprint arXiv:2407.12883},
  year    = {2024}
}

@article{abdallah2026mmbright,
  title   = {{MM-BRIGHT}: A Multi-Task Multimodal Benchmark for
             Reasoning-Intensive Retrieval},
  author  = {Abdallah, Abdelrahman and Mounis, Mohamed Darwish and
             Abdalla, Mahmoud and Kasem, Mahmoud SalahEldin and
             Senussi, Mostafa Farouk and Mahmoud, Mohamed and
             Ali, Mohammed and Jatowt, Adam and Kang, Hyun-Soo},
  journal = {arXiv preprint arXiv:2601.09562},
  year    = {2026}
}

@article{abdallah2026tempo,
  title   = {{TEMPO}: Temporal Reasoning Benchmark for Retrieval},
  author  = {Abdallah, Abdelrahman and Jatowt, Adam},
  journal = {arXiv preprint},
  year    = {2026}
}

% ============================================================
% REASONING-ENHANCED RETRIEVERS
% ============================================================

@article{shao2025reasonir,
  title   = {{ReasonIR}: Training Retrievers for Reasoning Tasks},
  author  = {Shao, Ruoqi and Qiao, Rui and Kishore, Vivek and
             Muennighoff, Niklas and Lin, Xi Victoria and Rus, Daniel and
             Low, Bryan Kian Hsiang and Min, Sewon and Yih, Wen-tau and
             Koh, Pang Wei and others},
  journal = {arXiv preprint arXiv:2504.20595},
  year    = {2025}
}

@article{das2025rader,
  title   = {{RaDeR}: Retrieval-Augmented Dense Retriever},
  author  = {Das, Rajarshi and others},
  journal = {arXiv preprint},
  year    = {2025}
}

@article{long2025diver,
  title   = {{DIVER}: A Multi-Stage Approach for Reasoning-Intensive
             Information Retrieval},
  author  = {Long, Dingkun and others},
  journal = {arXiv preprint arXiv:2508.07995},
  year    = {2025}
}

% ============================================================
% QUERY EXPANSION / REWRITING
% ============================================================

@article{wang2023query2doc,
  title   = {Query2doc: Query Expansion with Large Language Models},
  author  = {Wang, Liang and Yang, Nan and Wei, Furu},
  journal = {arXiv preprint arXiv:2303.07678},
  year    = {2023}
}

@article{gao2022hyde,
  title   = {Precise Zero-Shot Dense Retrieval without Relevance Labels},
  author  = {Gao, Luyu and Ma, Xueguang and Lin, Jimmy and Callan, Jamie},
  journal = {arXiv preprint arXiv:2212.10496},
  year    = {2022}
}

@article{lei2025thinkqe,
  title   = {{ThinkQE}: Query Expansion with Chain-of-Thought Reasoning},
  author  = {Lei, Wenhan and others},
  journal = {arXiv preprint},
  year    = {2025}
}

@article{ma2023rewrite,
  title   = {Query Rewriting for Retrieval-Augmented Large Language Models},
  author  = {Ma, Xinbei and Gong, Yeyun and He, Pengcheng and
             Zhao, Hai and Duan, Nan},
  journal = {arXiv preprint arXiv:2305.14283},
  year    = {2023}
}

@inproceedings{chen2024reinvoke,
  title     = {Re-Invoke: Tool Retrieval via Reversed Instructions},
  author    = {Chen, Yanfei and Yoon, Jinsung and Lee, Chanyeol and others},
  booktitle = {arXiv preprint arXiv:2408.01875},
  year      = {2024}
}

@article{yu2020conqrr,
  title   = {Few-Shot Generative Conversational Query Rewriting},
  author  = {Yu, Shi and Liu, Jiahua and Yang, Jingqing and Xu, Chenyan and
             Yu, Huan and Liu, Zhiyuan and Sun, Maosong},
  journal = {arXiv preprint},
  year    = {2020}
}

@article{mao2023convgqr,
  title   = {{ConvGQR}: Generative Query Reformulation for Conversational
             Search},
  author  = {Mao, Kelong and Dou, Zhicheng and Mo, Fengran and
             Wen, Jian-Yun and others},
  journal = {arXiv preprint arXiv:2305.15645},
  year    = {2023}
}

% ============================================================
% RL FOR QUERY OPTIMIZATION
% ============================================================

@article{jiang2025deepretrieval,
  title   = {{DeepRetrieval}: Hacking Real Search Engines and Retrievers
             with Large Language Models via Reinforcement Learning},
  author  = {Jiang, Pengcheng and Lin, Jiacheng and Cao, Lang and
             Tian, Runchu and Kang, SeongKu and Wang, Zifeng and
             Sun, Jimeng and Han, Jiawei},
  journal = {arXiv preprint arXiv:2503.00223},
  year    = {2025}
}

@article{cha2025rlqr,
  title   = {Annotation-Free Reinforcement Learning Query Rewriting via
             Verifiable Search Reward},
  author  = {Cha, Sungguk and others},
  journal = {arXiv preprint arXiv:2507.23242},
  year    = {2025}
}

@article{convr1,
  title   = {{ConvSearch-R1}: Enhancing Query Reformulation for
             Conversational Search with Reasoning via Reinforcement Learning},
  author  = {others},
  journal = {arXiv preprint arXiv:2505.15776},
  year    = {2025}
}

@article{nguyen2025rlecom,
  title   = {{RL}-based Query Rewriting with Distilled {LLM} for Online
             E-Commerce Systems},
  author  = {Nguyen, Duc Anh and others},
  journal = {arXiv preprint arXiv:2501.18056},
  year    = {2025}
}

% ============================================================
% LLM / RLHF
% ============================================================

@article{ouyang2022rlhf,
  title   = {Training Language Models to Follow Instructions with Human
             Feedback},
  author  = {Ouyang, Long and Wu, Jeff and Jiang, Xu and Almeida, Diogo and
             Wainwright, Carroll and Mishkin, Pamela and Zhang, Chong and
             Agarwal, Sandhini and Agarwal, Katarina Slama, Alex and
             Gray, Scott and others},
  journal = {Advances in Neural Information Processing Systems},
  volume  = {35},
  pages   = {27730--27744},
  year    = {2022}
}

@article{deepseek2025r1,
  title   = {{DeepSeek-R1}: Incentivizing Reasoning Capability in {LLM}s
             via Reinforcement Learning},
  author  = {DeepSeek-AI and Guo, Daya and Yang, Dejian and Zhang, Haowei
             and others},
  journal = {arXiv preprint arXiv:2501.12948},
  year    = {2025}
}

@article{shao2024grpo,
  title   = {DeepSeekMath: Pushing the Limits of Mathematical Reasoning in
             Open Language Models},
  author  = {Shao, Zhihong and Wang, Peiyi and Zhu, Qihao and Xu, Runxin
             and Song, Junxiao and Bi, Xiao and Zhang, Haowei and Zhang,
             Mingchuan and Li, YK and Wu, Y and others},
  journal = {arXiv preprint arXiv:2402.03300},
  year    = {2024}
}

@article{qwen2025,
  title   = {{Qwen2.5} Technical Report},
  author  = {Qwen Team},
  journal = {arXiv preprint arXiv:2412.15115},
  year    = {2025}
}

@inproceedings{wei2022chain,
  title     = {Chain-of-Thought Prompting Elicits Reasoning in Large
               Language Models},
  author    = {Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and
               Bosma, Maarten and Xia, Fei and Chi, Ed and Le, Quoc V and
               Zhou, Denny},
  booktitle = {Advances in Neural Information Processing Systems},
  volume    = {35},
  pages     = {24824--24837},
  year      = {2022}
}

% ============================================================
% RERANKING
% ============================================================

@article{sun2023rankgpt,
  title   = {Is {ChatGPT} Good at Search? Investigating Large Language
             Models as Re-Ranking Agents},
  author  = {Sun, Weiwei and Yan, Lingyong and Ma, Xinyu and Wang, Shuaiqiang
             and Ren, Pengjie and Chen, Zhumin and Yin, Dawei and Ren, Zhaochun},
  journal = {arXiv preprint arXiv:2304.09542},
  year    = {2023}
}

@article{weller2025rank1,
  title   = {{Rank1}: Test-Time Compute for Reranking},
  author  = {Weller, Orion and others},
  journal = {arXiv preprint arXiv:2502.18418},
  year    = {2025}
}

@article{zhuang2025rankr1,
  title   = {{RankR1}: Enhancing Reranking with Reasoning via
             Reinforcement Learning},
  author  = {Zhuang, Shengyao and others},
  journal = {arXiv preprint},
  year    = {2025}
}

@article{abdallah2025dear,
  title   = {{DEAR}: Dense Retrieval with Adaptive Reranking},
  author  = {Abdallah, Abdelrahman and Jatowt, Adam},
  journal = {arXiv preprint},
  year    = {2025}
}

% ============================================================
% MULTIMODAL EMBEDDING MODELS
% ============================================================

@inproceedings{radford2021clip,
  title     = {Learning Transferable Visual Models from Natural Language
               Supervision},
  author    = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and
               Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and
               Sastry, Girish and Askell, Amanda and Mishkin, Pamela and
               Clark, Jack and others},
  booktitle = {Proceedings of ICML},
  pages     = {8748--8763},
  year      = {2021}
}

@article{zhai2023siglip,
  title   = {Sigmoid Loss for Language Image Pre-Training},
  author  = {Zhai, Xiaohua and Mustafa, Basil and Kolesnikov, Alexander and
             Beyer, Lucas},
  journal = {arXiv preprint arXiv:2303.15343},
  year    = {2023}
}

@article{nomic2024vision,
  title   = {Nomic Embed: Training a Reproducible Long Context Text Embedder},
  author  = {Nussbaum, Zach and Morris, John X. and Duderstadt, Brandon and
             Mulyar, Andriy},
  journal = {arXiv preprint arXiv:2402.01613},
  year    = {2024}
}

@article{jiang2024vlm2vec,
  title   = {{VLM2Vec}: Training Vision-Language Models for Massive
             Multimodal Embedding Tasks},
  author  = {Jiang, Ziyan and Meng, Rui and Yang, Xinyi and Yavuz, Semih
             and Zhou, Yingbo and Chen, Wenhu},
  journal = {arXiv preprint arXiv:2410.05160},
  year    = {2024}
}

@article{zhang2024gme,
  title   = {{GME}: Improving Universal Multimodal Retrieval by Multimodal
             {LLM}s},
  author  = {Zhang, Xin and Zhang, Yanzhao and Xie, Wen and Li, Mingxin and
             Dai, Ziqi and Long, Dingkun and Xie, Pengjun and Zhang, Meishan
             and Li, Wenjie and Zhang, Min},
  journal = {arXiv preprint arXiv:2412.16855},
  year    = {2024}
}

@article{li2026qwen3vl,
  title   = {{Qwen3-VL-Embedding} and {Qwen3-VL-Reranker}: A Unified
             Framework for State-of-the-Art Multimodal Retrieval and Ranking},
  author  = {Li, Mingxin and Zhang, Yanzhao and Long, Dingkun and
             Chen, Keqin and others},
  journal = {arXiv preprint arXiv:2601.04720},
  year    = {2026}
}

@article{koukounas2024jinaclip,
  title   = {{Jina CLIP}: Your {CLIP} Model is Also Your Text Retriever},
  author  = {Koukounas, Andreas and others},
  journal = {arXiv preprint arXiv:2405.20204},
  year    = {2024}
}

% ============================================================
% VISUAL DOCUMENT RETRIEVAL
% ============================================================

@inproceedings{faysse2024colpali,
  title     = {{ColPali}: Efficient Document Retrieval with Vision Language
               Models},
  author    = {Faysse, Manuel and Sibille, Hugues and Wu, Tony and
               Omrani, Bilel and Viaud, Gautier and Hudelot, C{\'e}line and
               Colombo, Pierre},
  booktitle = {arXiv preprint arXiv:2407.01449},
  year      = {2024}
}

@article{ma2024dse,
  title   = {Unifying Multimodal Retrieval via Document Screenshot Embedding},
  author  = {Ma, Xueguang and Lin, Jimmy and Zhang, Minghan and Lin, Sheng-Chieh},
  journal = {arXiv preprint arXiv:2406.11251},
  year    = {2024}
}

@article{yu2024visrag,
  title   = {{VisRAG}: Vision-based Retrieval-Augmented Generation on
             Multi-Modality Documents},
  author  = {Yu, Shi and Tang, Chaoyue and Xu, Bokai and Cui, Junbo and
             Ran, Junhao and Yan, Yukun and Liu, Zhenghao and Wang, Shuo and
             Han, Xu and Liu, Zhiyuan and Sun, Maosong},
  journal = {arXiv preprint arXiv:2410.10594},
  year    = {2024}
}
